Designing Collaborative AI-Driven Workflows for Scientific Software Engineering

Agentic artificial intelligence systems can carry out a broad range of tasks in software engineering and scientific research, from writing and translating code to running workflows for data analysis and visualization. In scientific computing, the difficulty is verifying that agent-generated code is both correct and understandable to teams whose members bring different areas of expertise. We therefore argue that these systems are best used within collaborative team structures rather than as full automation. In the workflows we propose, domain experts write the specification and plan, and agents operate under a deterministic orchestration pattern to write the target code. Each stage ends with a numerical comparison against the reference code and requires human review and approval before the next begins. We evaluate these workflows on the translation of a large high-energy physics application from Fortran to C++, running the same task under different orchestrators, design patterns, and models. Across fourteen experiments, a simple author--reviewer loop with enforced limits completed a comparable number of files to a multi-agent workflow at about one-third of the cost per file.

==> eval_colors.tex <==
%% GENERATED by evals/analysis/generate_graphs.py -- DO NOT HAND-EDIT.
%% Regenerate with: python3 analysis/generate_graphs.py
%% Numbers are identical to analysis/summary_tables.md.
%% \input this in the preamble (or paste into jss-submission.sty).
%% The hex values below are hand-muted (blended toward evalInk) to match the
%% grayscale-leaning palette of the hand-drawn figures; re-apply this blend
%% after regenerating from generate_graphs.py, which writes saturated originals.
%% COLORBLIND FIX (2026-10-06): evalAqua and evalGreen (renamed evalIndigo)
%% were re-picked -- verified under simulated protanopia/deuteranopia/
%% tritanopia (Machado 2009 matrices) to keep every pair in the
%% blue/orange/aqua trio (fig_eval panels a,b,d,e + fig_decision) and the
%% red/indigo/magenta trio (fig_eval panel f) at >=60 sRGB-distance under all
%% three deficiencies -- the old evalAqua vs evalOrange and evalRed vs
%% evalGreen pairs both dropped below ~50 (red/green below 30) under
%% deuteranopia/protanopia. Port the same two swatches into
%% generate_graphs.py's CAT/MODULE_COLOR dicts (saturated originals, pre-mute)
%% next time this file is regenerated, or the fix will be silently reverted.
\definecolor{evalBlue}{HTML}{386AA6}
\definecolor{evalOrange}{HTML}{B5603D}
\definecolor{evalAqua}{HTML}{3DAF9B}
\definecolor{evalViolet}{HTML}{4D4288}
\definecolor{evalYellow}{HTML}{B7851B}
\definecolor{evalMagenta}{HTML}{B46C86}
\definecolor{evalIndigo}{HTML}{27309B}
\definecolor{evalRed}{HTML}{B04C4A}
\definecolor{evalVioletLight}{HTML}{706AB3}
\definecolor{evalGrid}{HTML}{E1E0D9}
\definecolor{evalAxis}{HTML}{C3C2B7}
\definecolor{evalInk}{HTML}{52514E}
\definecolor{evalInkStrong}{HTML}{0B0B0B}
\definecolor{evalSurface}{HTML}{FCFCFB}
\definecolor{evalOrd0}{HTML}{86B6EF}
\definecolor{evalOrd1}{HTML}{3987E5}
\definecolor{evalOrd2}{HTML}{1C5CAB}

